Search for dark matter in events with a hadronically decaying vector boson and missing transverse momentum in $pp$ collisions at $\sqrt{s} = 13$ TeV with the ATLAS detector

A search for dark matter (DM) particles produced in association with a hadronically decaying vector boson is performed using $pp$ collision data at a centre-of-mass energy of $\sqrt{s}=13$ TeV corresponding to an integrated luminosity of 36.1 fb$^{-1}$, recorded by the ATLAS detector at the Large Hadron Collider. This analysis improves on previous searches for processes with hadronic decays of $W$ and $Z$ bosons in association with large missing transverse momentum (mono-$W/Z$ searches) due to the larger dataset and further optimization of the event selection and signal region definitions. In addition to the mono-$W/Z$ search, the as yet unexplored hypothesis of a new vector boson $Z^\prime$ produced in association with dark matter is considered (mono-$Z^\prime$ search). No significant excess over the Standard Model prediction is observed. The results of the mono-$W/Z$ search are interpreted in terms of limits on invisible Higgs boson decays into dark matter particles, constraints on the parameter space of the simplified vector-mediator model and generic upper limits on the visible cross sections for $W/Z$+DM production. The results of the mono-$Z^\prime$ search are shown in the framework of several simplified-model scenarios involving DM production in association with the $Z^\prime$ boson.

==> EXOT-2016-23-PAPER-auxmat.tex <==

\begin{figure}[!hp]
\centering
\includegraphics[width=1.\textwidth]{pfigures/auxiliary/event_display_Merged0bESDEvent.png}
\caption{Candidate event for dark matter production in association with a hadronically decaying vector boson. The dashed line shows the direction of the missing transverse momentum, which has a magnitude of about 287~\GeV. The green and yellow bars indicate energy deposits in the liquid argon and scintillating-tile calorimeters, respectively. From these deposits one large-radius ($R=1.0$) jet is identified with transverse momentum of 269~\GeV\ and an invariant mass of 85~\GeV.
\label{fig:event_display_merged}
}
\end{figure}
\newpage

\begin{figure}[!htbp]
\centering
\includegraphics[width=1.\textwidth]{pfigures/auxiliary/event_display_WZMET_ev2_resolved_v2.png}
\caption{Candidate event for dark matter production in association with a hadronically decaying vector boson. The dashed line shows the direction of the missing transverse momentum, which has a magnitude of about 620~\GeV. The green and yellow bars indicate energy deposits in the liquid argon and scintillating-tile calorimeters, respectively. From these deposits two small-radius ($R=0.4$) jets are identified with transverse momenta of 388 and 30~\GeV. The invariant mass of the dijet system is 80~\GeV.
\label{fig:event_display_resolved}
}
\end{figure}
\newpage

\begin{figure}[!htbp]
\begin{center}
\subfigure[\label{fig:2dLimitPlots_c}]{\includegraphics[width=0.49\textwidth]{pfigures/auxiliary/monoWZ/monoW95CLsLimitPlot}}
\subfigure[\label{fig:2dLimitPlots_d}]{\includegraphics[width=0.49\textwidth]{pfigures/auxiliary/monoWZ/monoZ95CLsLimitPlot}}
\caption{
\label{fig:2dLimitPlots} 
Exclusion contours at 95\% CL in the plane of the DM particle mass, $m_{\chi}$, and the mediator
mass, $m_{Z'}$, for the individual (a) mono-$W$ and (b) mono-$Z$ channels in the frame of the simplified vector-mediator model with Dirac DM particles and couplings \gsm~=~0.25 and \gdm~=~1.
The black solid (dashed) curve shows the median of the observed (expected) limit. The dotted magenta curve corresponds to the set of points for which the expected relic density is consistent with the WMAP~\cite{WMAP} and Planck~\cite{Planck_relic} measurements ($\Omega h^2 = 0.12$), as computed with MadDM~\cite{MadDM}. The region on the right of the curve corresponds to higher predicted relic abundance than these measurements.
}
\end{center}
\end{figure}


\begin{table}[!htbp]
\centering
\caption{\label{tab:monowzmu} Theoretical cross section for $\sigma(pp \rightarrow W/Z + \chi \chi) \times \mathcal{B}(W/Z \rightarrow qq)$ at $\sqrt{s}=$~13~\TeV\ for each of the simplified vector-mediator model signal points. Also shown are the observed limits at 95\% CL on the signal strength $\mu$ for an integrated luminosity of 36.1~fb$^{-1}$ together with expectations varied up and down by one standard deviation. The prediction at a given signal point are obtained either from simulation (`(S)') or from interpolation (`(I)').}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{rr cr rrrr || rr cr rrrr}
\hline\hline
$m_{Z'}$         & $m_{\chi}$                 &    & 
$\sigma\times \mathcal{B}$     & \multicolumn{4}{c||}{95\% CL exclusion limit on $\mu$}&
$m_{Z'}$         & $m_{\chi}$                 &    & 
$\sigma\times \mathcal{B}$     & \multicolumn{4}{c}{95\% CL exclusion limit on $\mu$}\\

$\lbrack$\GeV$\rbrack$ &  $\lbrack$\GeV$\rbrack$ &   & 
[pb]  & Observed  & Expected &       +1$\sigma$ &   -1$\sigma$ &
$\lbrack$\GeV$\rbrack$ &  $\lbrack$\GeV$\rbrack$ &   & 
[pb]  & Observed  & Expected &       +1$\sigma$ &   -1$\sigma$ \\ 

 \hline


  10 &   1 & (S) & 455.75 & 0.06 & 0.07 & 0.09 & 0.05&
 900 &   1 & (S) & 0.1313 & 1.33 & 1.50 & 2.09 & 1.08  \\
  10 &  10 & (S) & 4.6338 & 2.16 & 2.17 & 3.02 & 1.56&
 900 &  50 & (I) & 0.1313 & 1.33 & 1.50 & 2.09 & 1.08\\

  10 &  50 & (S) & 0.2704 & 4.02 & 5.88 & 8.18 & 4.24&
 900 & 100 & (I) & 0.1312 & 1.33 & 1.50 & 2.09 & 1.08\\
  10 & 150 & (S) & 0.0258 & 11.55 & 13.83 & 19.25 & 9.97&
 900 & 150 & (I) & 0.1309 & 1.34 & 1.51 & 2.10 & 1.09\\
 100 &   1 & (S) & 18.0005 & 0.22 & 0.19 & 0.27 & 0.14&
 900 & 200 & (I) & 0.1302 & 1.34 & 1.52 & 2.11 & 1.09\\

 100 &  10 & (S)& 17.9640 & 0.22 & 0.20 & 0.28 & 0.15&
 900 & 250 & (I) & 0.1284 & 1.36 & 1.54 & 2.14 & 1.11\\
 100 &  45 & (I)& 13.7806 & 0.29 & 0.25 & 0.35 & 0.18&
 900 & 300 & (I) & 0.1248 & 1.40 & 1.58 & 2.20 & 1.14\\
  95 &  50 & (S)& 1.5237 & 1.82 & 1.97 & 2.74 & 1.42&
 900 & 350 & (I) & 0.1175 & 1.49 & 1.68 & 2.34 & 1.21\\
  
 200 &   1 & (S)& 5.4503 & 0.43 & 0.39 & 0.55 & 0.28&
 900 & 400 & (I) & 0.1011 & 1.73 & 1.95 & 2.72 & 1.41\\
 200 &  50 & (I)& 5.3816 & 0.44 & 0.40 & 0.55 & 0.29&
 900 & 445 & (I) & 0.0459 & 3.82 & 4.30 & 5.99 & 3.10\\

 200 &  95 & (I) & 3.4410 & 0.68 & 0.62 & 0.86 & 0.45&
1000 &  1 &  (S) & 0.0935 & 1.84 & 1.76 & 2.45 & 1.27\\
 
 300 &   1 & (S)& 2.4337 & 0.70 & 0.53 & 0.73 & 0.38&
1000 & 50 &  (I) & 0.0935 & 1.84 & 1.76 & 2.45 & 1.27\\

 300 &  50 & (S) & 2.4194 & 0.34 & 0.32 & 0.45 & 0.23&
1000 & 100 & (I) & 0.0934 & 1.84 & 1.76 & 2.45 & 1.27\\
 300 & 100 & (I)& 2.3239 & 0.74 & 0.55 & 0.77 & 0.40&
1000 & 150 & (S) & 0.0927 & 1.44 & 1.72 & 2.40 & 1.24\\
 300 & 145 & (I)& 1.3490 & 1.27 & 0.95 & 1.32 & 0.69&
1000 & 200 & (I)& 0.0930 & 1.85 & 1.77 & 2.46 & 1.27\\
 295 & 150 & (S)& 0.3590 & 1.90 & 2.16 & 3.01 & 1.56&
1000 & 250 & (I)& 0.0922 & 1.86 & 1.78 & 2.48 & 1.28\\


 400 &   1 &  (S) & 1.2052 & 0.42 & 0.53 & 0.73 & 0.38&
1000 & 300 &  (I) & 0.0906 & 1.89 & 1.81 & 2.52 & 1.31\\
 400 &  50 &  (I) & 1.2042 & 0.42 & 0.53 & 0.73 & 0.38&
1000 & 350 & (I)& 0.0877 & 1.96 & 1.87 & 2.61 & 1.35\\
 400 & 100 &  (I) & 1.1890 & 0.42 & 0.53 & 0.74 & 0.38&
1000 & 400 & (I)& 0.0821 & 2.09 & 2.00 & 2.79 & 1.44\\
 400 & 150 &  (I) & 1.1027 & 0.46 & 0.57 & 0.80 & 0.41&
1000 & 450 & (I)& 0.0700 & 2.45 & 2.35 & 3.27 & 1.69\\
 400 & 195 &  (I) & 0.5856 & 0.86 & 1.08 & 1.51 & 0.78&
1000 & 495 & (I)& 0.0313 & 5.49 & 5.25 & 7.31 & 3.79\\


 500 &   1 &  (S) & 0.6897 & 0.59 & 0.56 & 0.78 & 0.40&
 995 & 500 & (S)& 0.0195 & 8.09 & 7.75 & 10.79 & 5.59\\
 500 &  50 &  (I) & 0.6895 & 0.59 & 0.56 & 0.78 & 0.40&
2000 &   1 & (S)& 0.0062 & 12.96 & 13.12 & 18.26 & 9.45\\
 500 & 100 &  (I) & 0.6860 & 0.59 & 0.56 & 0.78 & 0.40&
2000 &  50 & (I)& 0.0062 & 12.96 & 13.12 & 18.26 & 9.45\\
 500 & 150 &  (I) & 0.6689 & 0.60 & 0.58 & 0.80 & 0.42&
2000 & 100 & (I)& 0.0062 & 12.96 & 13.12 & 18.26 & 9.45\\
 500 & 200 &  (I) & 0.6062 & 0.67 & 0.64 & 0.89 & 0.46&
2000 & 150 & (I)& 0.0062 & 12.96 & 13.12 & 18.26 & 9.45\\
 500 & 245 &  (I) & 0.3056 & 1.32 & 1.26 & 1.76 & 0.91&
2000 & 200 & (I)& 0.0062 & 12.96 & 13.12 & 18.26 & 9.46\\


 600 &   1 &  (S) & 0.4276 & 0.76 & 0.87 & 1.21 & 0.63&
2000 & 250 & (I)& 0.0062 & 12.97 & 13.13 & 18.27 & 9.46\\
 600 &  50 &  (I) & 0.4275 & 0.76 & 0.87 & 1.21 & 0.63&
2000 & 300 & (I)& 0.0062 & 12.98 & 13.14 & 18.29 & 9.47\\
 600 & 100 &  (I) & 0.4265 & 0.76 & 0.87 & 1.22 & 0.63&
2000 & 350 & (I)& 0.0062 & 13.00 & 13.16 & 18.31 & 9.48\\
 600 & 150 &  (I) & 0.4217 & 0.77 & 0.88 & 1.23 & 0.64&
2000 & 400 & (I)& 0.0061 & 13.03 & 13.19 & 18.36 & 9.50\\
 600 & 200 &  (I) & 0.4066 & 0.80 & 0.92 & 1.28 & 0.66&
2000 & 450 & (I)& 0.0061 & 13.07 & 13.24 & 18.42 & 9.54\\
 600 & 250 &  (I) & 0.3621 & 0.90 & 1.03 & 1.43 & 0.74&
2000 & 500 & (I)& 0.0061 & 13.14 & 13.30 & 18.51 & 9.59\\
 600 & 295 &  (I) & 0.1761 & 1.85 & 2.12 & 2.95 & 1.53&
2000 & 500 & (S)& 0.0058 & 13.80 & 13.56 & 18.87 & 9.77\\


 700 &   1 &  (S) & 0.2787 & 1.26 & 1.00 & 1.39 & 0.72&
2000 & 550 & (I)& 0.0060 & 13.23 & 13.40 & 18.65 & 9.65\\
 700 &  50 &  (I) & 0.2787 & 1.26 & 1.00 & 1.39 & 0.72&
2000 & 600 & (I)& 0.0060 & 13.36 & 13.53 & 18.83 & 9.75\\
 700 & 100 &  (I) & 0.2783 & 1.26 & 1.00 & 1.39 & 0.72&
2000 & 650 & (I)& 0.0059 & 13.55 & 13.72 & 19.09 & 9.89\\
 700 & 150 &  (I) & 0.2767 & 1.26 & 1.01 & 1.40 & 0.73&
2000 & 750 & (I)& 0.0056 & 14.19 & 14.37 & 20.00 & 10.35\\
 700 & 200 &  (I) & 0.2719 & 1.29 & 1.02 & 1.43 & 0.74&
2000 & 800 & (I)& 0.0054 & 14.76 & 14.94 & 20.80 & 10.77\\
 700 & 250 &  (I) & 0.2597 & 1.35 & 1.07 & 1.49 & 0.77&
2000 & 850 & (I)& 0.0051 & 15.66 & 15.86 & 22.07 & 11.43\\
 700 & 300 &  (I) & 0.2281 & 1.53 & 1.22 & 1.70 & 0.88&
2000 & 900 & (I)& 0.0046 & 17.30 & 17.51 & 24.37 & 12.62\\
 700 & 345 &  (I) & 0.1079 & 3.24 & 2.58 & 3.59 & 1.86&
2000 & 950 & (I)& 0.0038 & 21.23 & 21.50 & 29.92 & 15.49\\

 800 &   1 &  (S) & 0.1885 & 1.33 & 1.18 & 1.65 & 0.85&
2000 & 995 & (I)& 0.0015 & 52.03 & 52.69 & 73.33 & 37.96\\
 800 &  50 &  (I) & 0.1885 & 1.33 & 1.19 & 1.65 & 0.85&
 & & & & & & & \\
 800 & 100 &  (I) & 0.1884 & 1.33 & 1.19 & 1.65 & 0.85&
 & & & & & & & \\
 800 & 150 &  (I) & 0.1877 & 1.34 & 1.19 & 1.66 & 0.86&
 & & & & & & & \\
 800 & 200 &  (I) & 0.1859 & 1.35 & 1.20 & 1.67 & 0.87&
 & & & & & & & \\
 800 & 250 &  (I) & 0.1816 & 1.38 & 1.23 & 1.71 & 0.89&
 & & & & & & & \\
 800 & 300 &  (I) & 0.1721 & 1.46 & 1.30 & 1.81 & 0.94&
 & & & & & & & \\
 800 & 350 &  (I) & 0.1495 & 1.68 & 1.49 & 2.08 & 1.08&
 & & & & & & & \\
 800 & 395 &  (I) & 0.0691 & 3.64 & 3.23 & 4.50 & 2.33&
 & & & & & & & \\

\hline\hline
\end{tabular}
}
\end{table}


\begin{table}[!htbp]
\centering
\caption{\label{tab:monoZp} 
The observed upper limits at 95\% CL on the cross section $\sigma(pp \rightarrow Z' + \chi \chi) \times \mathcal{B}(Z' \rightarrow qq)$ in pb for each of the \monoZprime model signal points, shown for an integrated luminosity of 36.1~fb$^{-1}$  at $\sqrt{s}=$~13~\TeV, together with expectations varied up and down by one standard deviation.}

\begin{tabular}{r | cccc| cccc}

\hline\hline
$m_{Z'}$ &
\multicolumn{8}{c}{Exclusion limit on $\sigma(pp \rightarrow Z' + \chi \chi) \times \mathcal{B}(Z' \rightarrow qq)$ [pb] at 95\% CL}\\	
\lbrack\GeV] & Observed& Expected& +1$\sigma$& -1$\sigma$&  Observed& Expected& +1$\sigma$& -1$\sigma$\\

\hline
& 
\multicolumn{4}{c|}{Dark fermion model, light scenario}&	
\multicolumn{4}{c}{Dark fermion model, heavy scenario}\\
\hline


80&	27&	15&	21&	11&	9.8&	6.0&	8.3&	4.3\\
90&	20.4&	10.9&	15.1&	7.8&	6.5&	3.6&	5.0&	2.6\\
100&	21.6&	11.2&	15.6&	8.1&	6.5&	3.3&	4.6&	2.4\\
110&	13.7&	8.5&	11.9&	6.1&	4.1&	2.9&	4.1&	2.1\\
120&	15.5&	10.1&	14.1&	7.3&	4.0&	2.6&	3.7&	1.9\\
130&	16.2&	8.5&	11.9&	6.1&	4.8&	2.6&	3.6&	1.8\\
140&	11.0&	8.4&	11.7&	6.0&	2.1&	1.5&	2.1&	1.1\\
150&	5.0&	6.0&	8.3&	4.3&	1.4&	1.3&	1.8&	0.9\\
160&	3.7&	4.8&	6.7&	3.4&	0.8&	1.0&	1.4&	0.7\\
170&	2.5&	3.8&	5.3&	2.8&	0.60&	0.83&	1.15&	0.60\\
180&	3.9&	4.1&	5.7&	3.0&	0.44&	0.70&	0.97&	0.50\\
190&	1.4&	2.9&	4.0&	2.1&	0.37&	0.68&	0.95&	0.49\\
200&	3.1&	2.9&	4.0&	2.1&	0.61&	0.53&	0.73&	0.38\\
250&	2.2&	1.6&	2.2&	1.1&	0.56&	0.25&	0.35&	0.18\\
300&	0.77&	0.88&	1.22&	0.63&	0.21&	0.16&	0.22&	0.11\\
350&	1.36&	0.59&	0.82&	0.42&	0.23&	0.09&	0.13&	0.07\\
400&	0.93&   0.49&   0.68&   0.35&	0.128&	0.059&	0.082&	0.042\\
450&	0.78&	0.35&	0.49&	0.25&	0.095&	0.045&	0.063&	0.033\\
500&    0.68&   0.35&   0.48&   0.25&   0.066&  0.033&  0.046&  0.024\\
\hline
& 
\multicolumn{4}{c|}{Dark Higgs model, light scenario}&	
\multicolumn{4}{c}{Dark Higgs model, heavy scenario}\\
	
\hline	
80&	5.5&	4.0&	5.6&	2.9&	1.0&	0.9&	1.3&	0.7\\
90&	5.6&	2.8&	3.9&	2.0&	1.3&	1.1&	1.5&	0.8\\
100&	5.1&	2.8&	3.8&	2.0&	1.4&	1.3&	1.8&	1.0\\
110&	3.6&	2.5&	3.5&	1.8&	2.4&	2.1&	2.9&	1.5\\
120&	2.4&	1.7&	2.4&	1.2&	2.2&	1.8&	2.6&	1.3\\
130&	2.4&	2.0&	2.7&	1.4&	2.1&	1.6&	2.2&	1.1\\
140&	1.9&	1.7&	2.3&	1.2&	1.5&	1.3&	1.8&	0.9\\
150&	2.0&	1.9&	2.6&	1.4&	1.0&	1.1&	1.5&	0.8\\
160&	1.3&	1.7&	2.4&	1.3&	0.50&	0.76&	1.06&	0.55\\
170&	0.7&	1.2&	1.6&	0.8&	0.58&	0.83&	1.15&	0.60\\
180&	1.0&	1.4&	1.9&	1.0&	0.47&	0.70&	0.98&	0.51\\
190&	1.1&	1.3&	1.9&	1.0&	0.29&	0.56&	0.78&	0.40\\
200&	1.6&	1.2&	1.7&	0.9&	0.60&	0.44&	0.61&	0.31\\
250&	1.88&	0.93&	1.29&	0.67&	0.31&	0.22&	0.30&	0.16\\
300&	0.94&	0.76&	1.06&	0.55&	0.15&	0.15&	0.21&	0.11\\
350&	1.40&	0.60&	0.84&	0.43&	0.18&	0.08&	0.12&	0.06\\
400&	1.16&	0.55&	0.76&	0.40&	0.102&	0.061&	0.086&	0.044\\
450&	1.10&	0.49&	0.69&	0.36&	0.087&	0.047&	0.066&	0.034\\
500&    0.80&   0.42&   0.58&   0.30&   0.064&  0.035&  0.048&  0.025\\

\hline\hline
\end{tabular}
\end{table}


\begin{figure}[!htbp]
\centering
\includegraphics[width=0.7\textwidth]{pfigures/auxiliary/cross_sections}     
\caption{Cross sections for selected parameters of the \monoWZ vector-mediator as well as the \monoZprime dark-fermion and dark-Higgs signal models, shown in dependence on the mediator mass $m_{Z'}.$ The kink at $m_{Z'}=$~125~\GeV\ for dark-Higgs models is due to the definition of the light and heavy dark-sector scenarios (see~Table~\ref{tab:mczprime}). The lines  are drawn to guide the eye.
\label{fig:xsections}
}
\end{figure}


\begin{table}[!htbp]
\caption{Cross sections at $\sqrt{s}=$~13~\TeV\ for the processes involving invisible Higgs boson decays, assuming \BHinv~=~100\%.}
\centering
\begin{tabular}{lr}
\hline
\hline
\multicolumn{1}{l}{Process}	&  \multicolumn{1}{r}{Cross section [fb]}\\
\hline

\multicolumn{1}{l}{$qq \rightarrow W^{+}H$}	&  \multicolumn{1}{r}{840}\\
\multicolumn{1}{l}{$qq \rightarrow W^{-}H$}	&  \multicolumn{1}{r}{533}\\
\multicolumn{1}{l}{$qq \rightarrow ZH$}	        &  \multicolumn{1}{r}{761}\\
\multicolumn{1}{l}{$gg \rightarrow ZH$}	        &  \multicolumn{1}{r}{123}\\
\multicolumn{1}{l}{$gg \rightarrow H$}	        &  \multicolumn{1}{r}{48580}\\
\multicolumn{1}{l}{VBF}       	                &  \multicolumn{1}{r}{3782}\\
\hline
\hline
\end{tabular}
\label{tab:xsections}
\end{table}



\newpage
\begin{table}[!htbp]
\centering
\caption{The product of acceptance and efficiency $(\mathcal{A} \times \varepsilon)_{\mathrm{total, category}}$ (in percent)  after the full event selection for the signal from invisible Higgs boson decays, shown separately for each event category in the signal and the sideband region.}
\begin{tabular}{l ccc|c }
\hline
\hline
Category& $VH$ & $ggH$& VBF& $VH$+$ggH$+VBF\\

\hline
\\
\multicolumn{5}{l}{Signal region}\\
\hline
Resolved, $0b$& 3.733& 0.234& 0.377& 0.347\\
Resolved, $1b$& 0.301& 0.010& 0.014& 0.019\\
Resolved, $2b$& 0.183& 0.002& 0.002& 0.007\\

Merged, $0b$-HP& 0.716& 0.010& 0.021& 0.032\\
Merged, $0b$-LP& 0.525& 0.048& 0.070& 0.063\\
Merged, $1b$-HP& 0.091& 0.001& 0.002& 0.003\\
Merged, $1b$-LP& 0.077& 0.006& 0.004& 0.008\\
Merged, $2b$&    0.048& 0.001& 0.000& 0.002\\
\hline

Total (signal region)& 5.674& 0.313& 0.491& 0.482\\

\hline
\\
\multicolumn{5}{l}{Sideband region}\\
\hline
Resolved, $0b$& 0.353& 0.097& 0.149& 0.108\\
Resolved, $1b$& 0.038& 0.005& 0.008& 0.007\\
Resolved, $2b$& 0.019& 0.001& 0.000& 0.001\\

Merged, $0b$-HP& 0.067& 0.018& 0.027& 0.020\\
Merged, $0b$-LP& 0.123& 0.026& 0.030& 0.029\\
Merged, $1b$-HP& 0.010& 0.002& 0.002& 0.002\\
Merged, $1b$-LP& 0.019& 0.004& 0.004& 0.005\\
Merged, $2b$&    0.016& 0.001& 0.001& 0.001\\
\hline

Total (sideband region) & 0.646& 0.154& 0.221& 0.173\\

\hline
\\
Total&    6.320& 0.467& 0.712& 0.656\\
\hline
\hline

\end{tabular}
\end{table}


\begin{figure}[!htbp]
\centering
\subfigure[]{\includegraphics[width=0.495\textwidth]{pfigures/auxiliary/acceptances_category_sr}}
\subfigure[]{\includegraphics[width=0.495\textwidth]{pfigures/auxiliary/acceptances_category_sb}}
\subfigure[]{\includegraphics[width=0.495\textwidth]{pfigures/auxiliary/acceptances_category_mzp_dfl}}
\subfigure[]{\includegraphics[width=0.495\textwidth]{pfigures/auxiliary/acceptances_category_mzp_dfh}}
\subfigure[]{\includegraphics[width=0.495\textwidth]{pfigures/auxiliary/acceptances_category_mzp_dhl}}
\subfigure[]{\includegraphics[width=0.495\textwidth]{pfigures/auxiliary/acceptances_category_mzp_dhh}}
\caption{The product of acceptance and efficiency $(\mathcal{A} \times \varepsilon)_{\mathrm{total, category}}$ in each event category of the zero-lepton region after the full event selection, shown in dependence on the mediator mass $m_{Z'}$ for the combined mono-$W$ and mono-$Z$ signal of the simplified vector-mediator model in (a) signal and (b) sideband regions, as well as for the \monoZprime signal from the (c) dark fermion model in the light dark sector, (d) dark fermion model in the heavy dark sector, (e) dark Higgs model in the light dark sector and (f) dark Higgs model in the heavy dark sector. The lines  are drawn to guide the eye.
\label{fig:ae}}
\end{figure}


\begin{table}[!htbp]
\centering
\caption{Cutflow for the simplified vector-mediator signal with $m_{\chi}=$~1~\GeV\ and $m_{Z'}=$~600~\GeV, shown for an integrated luminosity of 36.1~fb$^{-1}$ at $\sqrt{s}=$~13~\TeV\ separately for the combined \monoWZ search and individual mono-$W$ and mono-$Z$ channels. The uncertainty in the expected number of signal events is statistical only.}
\begin{tabular}{l r r r}
\hline\hline

Selection criteria &
Mono-$W/Z$ &
Mono-$W$ &
Mono-$Z$\\

 & 
channels & 
channel& 
channel\\

\hline  
\\ 
\multicolumn{4}{c}{Merged topology ($m_{\chi}=$~1~\GeV\ and $m_{Z'}=$~600~\GeV)}\\
\hline    
Preselection &
5230.18 &
3779.34 &
1450.85 \\

Trigger &
5070.97 &
3664.01 &
1406.96 \\

Lepton veto &
5069.65 &
3662.96 & 
1406.69 \\

$\mpt > \SI{30}{\GeV}$ &
4476.76 &
3259.06 &
1217.70 \\

$\min_{i\in \{1,2,3\}}\left[\Delta\phi(\vec{\met},j_i)\right]>$~20$^\textrm{o}$ &
4145.99 &
3016.91 & 
1129.08 \\

$\Delta\phi(\vec{\met}, \vec{\mpt}) < 90^{\circ}$ &
4110.77 &
2991.44 &
1119.33 \\

$\met > \SI{250}{\GeV}$ &
1543.72 &
1105.41 & 
438.31 \\

$\geq 1$ large-R jet &
1354.49 &
974.75 & 
379.74 \\

$\Delta\phi(\vec{\met}, J) > 120^{\circ}$ &
1344.00 &
967.06 &
376.94 \\

Non-associated $b$-jet veto &
1298.47 &
943.34 &
355.14 \\

$\SI{30}{\GeV} < m_{J} < \SI{250}{\GeV}$ &
1023.52 &
743.70 &
279.82 \\

$0 \leq b\text{-tagged jets}\leq 2$ &
1020.28 & 
742.45 &
277.83 \\
\hline
$W$/$Z$ mass window &
633.38 $\pm$ 3.08&
458.95 $\pm$ 2.96&
174.43 $\pm$ 0.86\\

Upper $W$/$Z$ mass side-band &
128.25 $\pm$ 1.77&
81.48 $\pm$ 1.53& 
46.77 $\pm$ 0.89\\

\hline\hline 
\\
\multicolumn{4}{c}{Resolved topology ($m_{\chi}=$~1~\GeV\ and $m_{Z'}=$~600~\GeV)}\\
\hline    

Preselection &
5230.18 &
3779.34 &
1450.85\\

Trigger &
5070.97 &
3664.01 &
1406.96 \\

Lepton veto &
5069.65 &
3662.96 &
1406.69 \\

$\mpt > \SI{30}{\GeV}$ &
3474.94 &
2516.49 & 
958.45 \\

$\min_{i\in \{1,2,3\}}\left[\Delta\phi(\vec{\met},j_i)\right]>$~20$^\textrm{o}$ &
3143.17 &
2274.20 & 
868.97 \\

$\Delta\phi(\vec{\met}, \mpt) < 90^{\circ}$ &
3106.28 &
2248.68 &
857.60 \\

$\met > \SI{150}{\GeV}$ &
2680.18 &
1935.27 &
744.91 \\

$\geq 2$ central jets &
2557.63 &
1844.07 &
713.56 \\
$\Delta\phi(\vec{\met}, jj) > 120^{\circ}$ &
2532.88 & 
1832.25 &
700.62 \\

Leading jet $\mpt > \SI{45}{\GeV}$ &
2476.07 &
1797.25 &
678.82 \\


$\Delta R < 1.4$ ($2b$: 1.25) &
1302.88 &
947.50 &
355.38 \\

$\sum_{j_1,j_2~(j_1,j_2,j_3)}p_{\text{T}}^{j} > 120~(150)~\GeV$ &
1296.39 & 
942.34 &
354.05 \\

$0 \leq b\text{-tagged jets}\leq 2$ &
1295.73 &
942.30 &
353.43 \\

$\SI{30}{\GeV} < m_{jj} < \SI{250}{\GeV}$ &
1279.99 &
931.70 &
348.30 \\
\hline

$W$/$Z$ mass window &
927.57 $\pm$ 0.94&
676.91 $\pm$ 0.13&
250.67 $\pm$ 0.93\\

Upper $W$/$Z$ mass side-band &
148.27 $\pm$ 0.30&
97.69 $\pm$ 0.06&
50.58 $\pm$ 0.30\\

\hline\hline
\end{tabular}
\end{table}




\begin{figure}[!htbp]
\begin{center}
\includegraphics[width=0.49\textwidth]{pfigures/auxiliary/monoWZ/monoV_0lep_0tag_merged_baseline_d2_XS}
\includegraphics[width=0.49\textwidth]{pfigures/auxiliary/monoWZ/monoV_0lep_1tag_merged_baseline_d2_XS}
\includegraphics[width=0.49\textwidth]{pfigures/auxiliary/monoWZ/monoV_0lep_2tag_merged_baseline_d2_XS}
\caption{\label{fig:auxiliary_d2}
The observed (dots) and expected (histograms) distribution of the large-$R$ jet substructure variable \DTwoBetaOne 
after applying all \monoWZ signal requirements except for the \DTwoBetaOne and mass window criteria, shown for the merged topology in the (a) $0b$, (b) $1b$ and (c) $2b$ final states. The plots are shown after the profile likelihood fit to the $\met$ distribution (with $\mu = 0$). The total background contribution before the fit to data is shown as a dotted blue line. The hatched area represents the total background uncertainty, defined by the post-fit nuisance parameters. The signal expectations for the simplified vector-mediator model with $m_{\chi}=1$~\GeV\ and $m_{Z'}=600$~\GeV\ (dashed red line) and for the invisible Higgs boson decays (dashed blue line) are shown for comparison. The inset at the bottom of each plot shows the ratio of the data to the total post-fit (dots) and pre-fit (dotted blue line) background expectation. 
}
\end{center}
\end{figure}



\begin{table}[!htbp]
\begin{center}
\caption{
\label{tab:event_yields_sideband}
The expected and observed numbers of events for an integrated luminosity of 36.1~fb$^{-1}$ and $\sqrt{s}=$~13~\TeV, shown separately in each \monoWZ mass sideband category. The background yields and uncertainties are shown after the profile likelihood fit to the data (with $\mu = 0$). The quoted background uncertainties include both the statistical and systematic contributions, while the uncertainty in the signal is statistical only.  The uncertainties in the total background can be smaller than in individual components due to anti-correlations of nuisance parameters.}
\resizebox{\linewidth}{!}{

\begin{tabular}{l cc cc c}
\hline\hline

& \multicolumn{5}{c}{Merged topology, $W/Z$ mass sideband}\\
Process &         
  $0b$-HP& 
  $0b$-LP& 
  $1b$-HP& 
  $1b$-LP& 
  $2b$ \\
  \hline
  \midrule
Vector-mediator model, \\
$m_{\chi}=$1~\GeV, $m_{Z'}=$200~\GeV &  
\phantom{00}116 $\pm$ 19\phantom{0}  &  
\phantom{00}178 $\pm$ 34\phantom{0}  &  
\phantom{0000}6.2 $\pm$ 1.7\phantom{00}  &  
\phantom{000}30.0 $\pm$ 8.9\phantom{00}  &  
\phantom{000}17.1 $\pm$ 3.1\phantom{00}  \\
$m_{\chi}=$1~\GeV, $m_{Z'}=$600~\GeV &  
\phantom{000}38.5 $\pm$ 3.1\phantom{00}  &  
\phantom{000}67.3 $\pm$ 3.9\phantom{00}  &  
\phantom{0000}6.4 $\pm$ 1.7\phantom{00}  &  
\phantom{000}10.1 $\pm$ 1.8\phantom{00}  &  
\phantom{0000}5.93 $\pm$ 0.69\phantom{00}  \\
\\
\multicolumn{6}{l}{Invisible Higgs boson decays ($m_H=$~125~\GeV, \BHinv~=~100\%)} \\
$VH$& 
\phantom{000}38.49 $\pm$ 0.84\phantom{00}& 
\phantom{000}70.1 $\pm$ 1.2\phantom{00}& 
\phantom{00}5.68 $\pm$ 0.38\phantom{}& 
\phantom{000}10.9 $\pm$ 0.5\phantom{00}& 
\phantom{00}9.36 $\pm$ 0.34\phantom{}\\
$ggH$& 
\phantom{00}323 $\pm$ 23\phantom{0}& 
\phantom{00}450 $\pm$ 26\phantom{0}& 
\phantom{000}39.3 $\pm$ 4.3\phantom{00}& 
\phantom{000}73.1 $\pm$ 6.3\phantom{0}& 
\phantom{000}13.8 $\pm$ 2.5\phantom{00}\\
VBF& 
\phantom{000}36.9 $\pm$ 2.8\phantom{00}& 
\phantom{000}41.0 $\pm$ 3.0\phantom{00}& 
\phantom{0000}2.82 $\pm$ 0.33\phantom{00}& 
\phantom{0000}5.90 $\pm$ 0.68\phantom{00}& 
\phantom{00}0.79 $\pm$ 0.13\phantom{}\\
\\

$W$+jets & 
\phantom{0}5010 $\pm$ 210 & 
\phantom{0}5400 $\pm$ 220 & 
\phantom{00}470 $\pm$ 60\phantom{0} & 
\phantom{00}646 $\pm$ 78\phantom{0} & 
\phantom{00}152 $\pm$ 22\phantom{0} \\
$Z$+jets & 
\phantom{0}7100 $\pm$ 300 & 
\phantom{0}7680 $\pm$ 320 & 
\phantom{00}822 $\pm$ 93\phantom{0} & 
\phantom{0}1030 $\pm$ 120 & 
\phantom{00}352 $\pm$ 20\phantom{0} \\
$t\bar{t}$ & 
\phantom{00}485 $\pm$ 50\phantom{0} & 
\phantom{00}896 $\pm$ 71\phantom{0} & 
\phantom{0}1348 $\pm$ 45\phantom{0} & 
\phantom{0}1947 $\pm$ 65\phantom{0} & 
\phantom{00}354 $\pm$ 27\phantom{0}\\
Single top-quark & 
\phantom{000}72.8 $\pm$ 8.6\phantom{00} & 
\phantom{00}131 $\pm$ 12\phantom{0} & 
\phantom{00}162 $\pm$ 11\phantom{0} & 
\phantom{00}225 $\pm$ 15\phantom{0} & 
\phantom{000}73.7 $\pm$ 6.1\phantom{00}\\
Diboson & 
\phantom{00}340 $\pm$ 55\phantom{0} & 
\phantom{00}474 $\pm$ 74\phantom{0} & 
\phantom{000}46.2 $\pm$ 7.3\phantom{00} & 
\phantom{000}69 $\pm$ 11\phantom{0} & 
\phantom{000}28.0 $\pm$ 4.6\phantom{00}\\
Multijet & 
\phantom{00}139 $\pm$ 123 & 
\phantom{00}152 $\pm$ 134 & 
\phantom{000}21 $\pm$ 15\phantom{0} & 
\phantom{000}21 $\pm$ 16\phantom{0} & 
\phantom{000}19 $\pm$ 22\phantom{0}\\
\hline
Total background & 
\phantom{}13140 $\pm$ 100 & 
\phantom{}14740 $\pm$ 110 & 
\phantom{0}2869 $\pm$ 44\phantom{0} & 
\phantom{0}3942 $\pm$ 51\phantom{0} & 
\phantom{00}979 $\pm$ 25\phantom{0}\\
Data & 
\phantom{}13205 \phantom{$\pm$ 000} & 
\phantom{}14673 \phantom{$\pm$ 000}& 
\phantom{0}2898 \phantom{$\pm$ 000}& 
\phantom{0}3982 \phantom{$\pm$ 000}& 
\phantom{00}966 \phantom{$\pm$ 000}\\
  
  
\hline\hline
Process & \multicolumn{5}{c}{Resolved topology, $W$/$Z$ mass sideband}\\
        & \multicolumn{2}{c}{$0b$}& \multicolumn{2}{c}{$1b$}& $2b$\\
  \midrule
Vector-mediator model, \\
$m_{\chi}=$1~\GeV, $m_{Z'}=$200~\GeV  & 
\multicolumn{2}{c}{\phantom{00}645 $\pm$ 45\phantom{0}} & 
\multicolumn{2}{c}{\phantom{000}45 $\pm$ 10\phantom{0}} &  
\phantom{000}11.7 $\pm$ 1.6\phantom{00} \\
$m_{\chi}=$1~\GeV, $m_{Z'}=$600~\GeV  & 
\multicolumn{2}{c}{\phantom{00}132.1 $\pm$ 6.3\phantom{00}} & 
\multicolumn{2}{c}{\phantom{000}12.9 $\pm$ 1.5\phantom{00}} &  
\phantom{00}3.29 $\pm$ 0.30\phantom{} \\
\\
\multicolumn{4}{l}{Invisible Higgs boson decays ($m_H=$~125~\GeV, \BHinv~=~100\%)} \\
$VH$& 
\multicolumn{2}{c}{\phantom{00}201.3 $\pm$ 2.9\phantom{00}}& 
\multicolumn{2}{c}{\phantom{000}21.64 $\pm$ 0.87\phantom{00}}& 
\phantom{00}11.09 $\pm$ 0.43\\
$ggH$& 
\multicolumn{2}{c}{\phantom{0}1702 $\pm$ 49\phantom{0}}& 
\multicolumn{2}{c}{\phantom{000}96 $\pm$ 14\phantom{0}}& 
\phantom{000}10.0 $\pm$ 1.9\phantom{00}\\
VBF& 
\multicolumn{2}{c}{\phantom{00}203.1 $\pm$ 6.5\phantom{00}}& 
\multicolumn{2}{c}{\phantom{000}10.64 $\pm$ 0.66\phantom{00}}& 
\phantom{00}0.40 $\pm$ 0.09\\
\\


$W$+jets & 
\multicolumn{2}{c}{\phantom{0}51000 $\pm$ 2200\phantom{}} & 
\multicolumn{2}{c}{\phantom{0}3260 $\pm$ 470} & 
\phantom{00}221 $\pm$ 38\phantom{0}\\
$Z$+jets & 
\multicolumn{2}{c}{\phantom{0}5400 $\pm$ 2400} & 
\multicolumn{2}{c}{\phantom{0}4580 $\pm$ 470} & 
\phantom{00}462 $\pm$ 25\phantom{0}\\
$t\bar{t}$ & 
\multicolumn{2}{c}{\phantom{0}5740 $\pm$ 390} & 
\multicolumn{2}{c}{\phantom{}14640 $\pm$ 440} & 
\phantom{00}756 $\pm$ 43\phantom{0}\\
Single top-quark & 
\multicolumn{2}{c}{\phantom{00}668 $\pm$ 44\phantom{0}} & 
\multicolumn{2}{c}{\phantom{0}1269 $\pm$ 79\phantom{0}} & 
\phantom{00}150 $\pm$ 11\phantom{0}\\
Diboson & 
\multicolumn{2}{c}{\phantom{0}1730 $\pm$ 260} & 
\multicolumn{2}{c}{\phantom{00}177 $\pm$ 26\phantom{0}} & 
\phantom{000}39.3 $\pm$ 6.8\phantom{00}\\
Multijet & 
\multicolumn{2}{c}{\phantom{0}6580 $\pm$ 920} & 
\multicolumn{2}{c}{\phantom{00}770 $\pm$ 280} & 
\phantom{00}279 $\pm$ 61\phantom{0}\\
\hline
Total background & 
\multicolumn{2}{c}{119660 $\pm$ 340\phantom{0}} & 
\multicolumn{2}{c}{24690 $\pm$ 160} & 
\phantom{0}1910 $\pm$ 42\phantom{0}\\
Data & 
\multicolumn{2}{c}{119676 \phantom {$\pm$ 0000}}  & 
\multicolumn{2}{c}{ 24645 \phantom{ $\pm$ 000}}  & 
\phantom{0}1904 \phantom{ $\pm$ 000} \\
\hline\hline
\end{tabular}
}
\end{center}
\end{table}




\begin{table}[!htbp]
\begin{center}
\caption{
\label{tab:event_yields_controlregion1lep_masswindow}
The expected and observed numbers of events for an integrated luminosity of 36.1~fb$^{-1}$ and $\sqrt{s}=$~13~\TeV, shown separately in each \monoWZ 1 lepton control region mass window category. The background yields and uncertainties are shown after the profile likelihood fit to the data (with $\mu = 0$). The quoted background uncertainties include both the statistical and systematic contributions.  The uncertainties in the total background can be smaller than in individual components due to anti-correlations of nuisance parameters.}
\resizebox{\linewidth}{!}{

\begin{tabular}{l cc cc c}
\hline\hline

& \multicolumn{3}{c}{Merged topology, 1 lepton control region $W/Z$ mass window}\\
Process &         
  $0b$  & 
  $1b$  & 
  $2b$ \\
  \hline
  \midrule

$W$+jets & 
 \num[group-digits=false, round-mode=figures,round-precision=4]{21899.79} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{868.29} & 
 \num[group-digits=false, round-mode=figures,round-precision=3]{2004.35} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{230.27}  & 
\phantom{0.}\num[group-digits=false, round-mode=figures,round-precision=3]{149.71} $\pm$ \phantom{0.}\num[group-digits=false, round-mode=figures,round-precision=2]{20.02}  \\
$Z$+jets & 
\phantom{00}\num[group-digits=false, round-mode=figures,round-precision=3]{608.04} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{25.93} & 
\phantom{.}\num[group-digits=false, round-mode=figures,round-precision=3]{60.34} $\pm$ \phantom{.}\num[group-digits=false, round-mode=figures,round-precision=2]{7.17} & 
\phantom{0}\num[group-digits=false, round-mode=figures,round-precision=3]{4.65} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{0.65} \\
$t\bar{t}$ & 
\phantom{0}\num[group-digits=false, round-mode=figures,round-precision=3]{3362.96} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{201.44} & 
\num[group-digits=false, round-mode=figures,round-precision=3]{2673.32} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{110.04} & 
\num[group-digits=false, round-mode=figures,round-precision=4]{105.58} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{8.77}\\
Single top-quark & 
\phantom{00}\num[group-digits=false, round-mode=figures,round-precision=3]{835.61} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{59.06} & 
\phantom{0}\num[group-digits=false, round-mode=figures,round-precision=3]{552.29} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{36.25} & 
\phantom{0}\num[group-digits=false, round-mode=figures,round-precision=3]{39.70} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{3.89}\\
Diboson & 
\phantom{0}\num[group-digits=false, round-mode=figures,round-precision=3]{1201.58} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{241.03} & 
\phantom{0}\num[group-digits=false, round-mode=figures,round-precision=3]{137.42} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{27.36} & 
\phantom{0}\num[group-digits=false, round-mode=figures,round-precision=3]{20.23} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{4.66}\\
Total background & 
\phantom{}\num[group-digits=false, round-mode=figures,round-precision=4]{27907.99} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{159.78} & 
\num[group-digits=false, round-mode=figures,round-precision=4]{5427.73} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{65.04} & 
\phantom{0.}\num[group-digits=false, round-mode=figures,round-precision=3]{319.88} $\pm$ \phantom{0.}\num[group-digits=false, round-mode=figures,round-precision=2]{14.95}\\
Data & 
\phantom{}27964 \phantom{$\pm$ 000} & 
\phantom{}5357 \phantom{$\pm$ 000}& 
\phantom{0.}312 \phantom{$\pm$ 0.00}\\
  
  
\hline\hline
Process & \multicolumn{3}{c}{Resolved topology, 1 lepton control region $W$/$Z$ mass window}\\
        & $0b$  & $1b$  & $2b$\\
  \midrule

$W$+jets & 
\num[group-digits=false, round-mode=figures,round-precision=4]{154575.51}  $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{6781.06} & 
\phantom{0}\num[group-digits=false, round-mode=figures,round-precision=3]{6293.71} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{876.81} & 
\phantom{0}\num[group-digits=false, round-mode=figures,round-precision=3]{1012.75} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{168.63}\\
$Z$+jets & 
\phantom{00}\num[group-digits=false, round-mode=figures,round-precision=3]{5926.90} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{ 249.01} & 
\phantom{00}\num[group-digits=false, round-mode=figures,round-precision=3]{293.98} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{31.85} & 
\phantom{0.}\num[group-digits=false, round-mode=figures,round-precision=3]{73.36} $\pm$ \phantom{.}\num[group-digits=false, round-mode=figures,round-precision=2]{4.48}\\
$t\bar{t}$ & 
\phantom{0}\num[group-digits=false, round-mode=figures,round-precision=3]{18752.44} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{1070.23} & 
\phantom{}\num[group-digits=false, round-mode=figures,round-precision=4]{17569.56} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{616.47} & 
\num[group-digits=false, round-mode=figures,round-precision=4]{10677.89} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{193.04}\\
Single top-quark & 
\phantom{00}\num[group-digits=false, round-mode=figures,round-precision=3]{3709.96} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{231.01} & 
\phantom{0}\num[group-digits=false, round-mode=figures,round-precision=3]{2523.81} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{158.71} & 
\phantom{00}\num[group-digits=false, round-mode=figures,round-precision=3]{967.68}  $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{52.56}\\
Diboson & 
\phantom{00}\num[group-digits=false, round-mode=figures,round-precision=3]{4261.17} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{861.28} & 
\phantom{00}\num[group-digits=false, round-mode=figures,round-precision=3]{278.85} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{50.60} & 
\phantom{00}\num[group-digits=false, round-mode=figures,round-precision=3]{116.59} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{26.53}\\
Total background & 
\num[group-digits=false, round-mode=figures,round-precision=4]{187225.97} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{500.51} & 
\num[group-digits=false, round-mode=figures,round-precision=4]{26959.91} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{168.16} & 
\num[group-digits=false, round-mode=figures,round-precision=4]{12848.27} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{108.81}\\
Data & 
187205 \phantom {$\pm$ 0000}  & 
26992 \phantom{ $\pm$ 000}  & 
12851 \phantom{ $\pm$ 000} \\
\hline\hline
\end{tabular}
}
\end{center}
\end{table}



\begin{table}[!htbp]
\begin{center}
\caption{
\label{tab:event_yields_controlregion1lep_sideband}
The expected and observed numbers of events for an integrated luminosity of 36.1~fb$^{-1}$ and $\sqrt{s}=$~13~\TeV, shown separately in each \monoWZ 1 lepton control region mass sideband category. The background yields and uncertainties are shown after the profile likelihood fit to the data (with $\mu = 0$). The quoted background uncertainties include both the statistical and systematic contributions.  The uncertainties in the total background can be smaller than in individual components due to anti-correlations of nuisance parameters.}
\resizebox{\linewidth}{!}{

\begin{tabular}{l cc cc c}
\hline\hline

& \multicolumn{3}{c}{Merged topology, 1 lepton control region $W/Z$ mass sideband}\\
Process &         
  $0b$  & 
  $1b$  & 
  $2b$ \\
  \hline
  \midrule

$W$+jets & 
 \num[group-digits=false, round-mode=figures,round-precision=4]{16188.40} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{692.73} & 
 \num[group-digits=false, round-mode=figures,round-precision=3]{1768.56} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{212.73} & 
 \phantom{0.}\num[group-digits=false, round-mode=figures,round-precision=3]{278.58} $\pm$ \phantom{0.}\num[group-digits=false, round-mode=figures,round-precision=2]{39.18}  \\
$Z$+jets & 
 \phantom{00}\num[group-digits=false, round-mode=figures,round-precision=3]{480.44} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{20.37} & 
 \phantom{.}\num[group-digits=false, round-mode=figures,round-precision=3]{56.45} $\pm$ \phantom{.}\num[group-digits=false, round-mode=figures,round-precision=2]{6.19} & 
 \num[group-digits=false, round-mode=figures,round-precision=4]{10.65} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{ 0.78} \\
$t\bar{t}$ & 
 \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=3]{2357.24} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{201.59}  & 
 \num[group-digits=false, round-mode=figures,round-precision=3]{5734.31} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{162.19}   & 
 \phantom{0.}\num[group-digits=false, round-mode=figures,round-precision=3]{602.07} $\pm$ \phantom{0.}\num[group-digits=false, round-mode=figures,round-precision=2]{ 37.85} \\
Single top-quark & 
 \phantom{00}\num[group-digits=false, round-mode=figures,round-precision=3]{439.15} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{38.77}  & 
 \num[group-digits=false, round-mode=figures,round-precision=4]{1012.23} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{67.58}  & 
 \phantom{0.}\num[group-digits=false, round-mode=figures,round-precision=3]{174.14} $\pm$ \phantom{0.}\num[group-digits=false, round-mode=figures,round-precision=2]{13.80} \\
Diboson & 
 \phantom{00}\num[group-digits=false, round-mode=figures,round-precision=2]{534.39}  $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{101.62}  & 
 \phantom{00}\num[group-digits=false, round-mode=figures,round-precision=2]{75.10} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{13.92} & 
 \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=3]{11.70} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{2.76} \\
Total background & 
\num[group-digits=false, round-mode=figures,round-precision=4]{19999.61} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{134.54} & 
\num[group-digits=false, round-mode=figures,round-precision=4]{8646.66}  $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{86.74} & 
\phantom{.}\num[group-digits=false, round-mode=figures,round-precision=4]{1077.15} $\pm$ \phantom{0.}\num[group-digits=false, round-mode=figures,round-precision=2]{28.38}\\
Data & 
\phantom{}  19983 \phantom{$\pm$ 000} & 
\phantom{}  8621 \phantom{$\pm$ 000}& 
\phantom{.}1076\phantom{$\pm$ .000}\\
  
  
\hline\hline
Process & \multicolumn{3}{c}{Resolved topology, 1 lepton control region $W$/$Z$ mass sideband}\\
        & $0b$  & $1b$  & $2b$\\
  \midrule

$W$+jets & 
 \num[group-digits=false, round-mode=figures,round-precision=3]{343430.73} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{16210.57}& 
 \num[group-digits=false, round-mode=figures,round-precision=3]{16654.31} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{2288.18} & 
 \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=3]{1539.99} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{245.90} \\
$Z$+jets & 
 \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=4]{13297.79} $\pm$ \phantom{00}\num[group-digits=false, round-mode=figures,round-precision=2]{579.12}  & 
 \phantom{00}\num[group-digits=false, round-mode=figures,round-precision=3]{791.67} $\pm$ \phantom{00}\num[group-digits=false, round-mode=figures,round-precision=2]{83.38} & 
 \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=4]{152.44} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{8.77} \\
$t\bar{t}$ & 
 \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=3]{20282.07} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{1259.32} & 
 \num[group-digits=false, round-mode=figures,round-precision=3]{50760.00}  $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{1506.05} & 
 \num[group-digits=false, round-mode=figures,round-precision=4]{29678.84} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{343.09} \\
Single top-quark & 
 \phantom{00}\num[group-digits=false, round-mode=figures,round-precision=3]{4098.16}  $\pm$ \phantom{00}\num[group-digits=false, round-mode=figures,round-precision=2]{241.34}  & 
 \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=3]{7271.06} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{440.63}  & 
 \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=3]{3179.58} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{180.81} \\
Diboson & 
 \phantom{00}\num[group-digits=false, round-mode=figures,round-precision=3]{3932.93}   $\pm$ \phantom{00}\num[group-digits=false, round-mode=figures,round-precision=2]{755.69} & 
 \phantom{00}\num[group-digits=false, round-mode=figures,round-precision=3]{350.72} $\pm$ \phantom{00}\num[group-digits=false, round-mode=figures,round-precision=2]{60.54}  & 
 \phantom{0.}\num[group-digits=false, round-mode=figures,round-precision=3]{49.74} $\pm$ \phantom{.}\num[group-digits=false, round-mode=figures,round-precision=2]{9.46} \\
Total background & 
\num[group-digits=false, round-mode=figures,round-precision=5]{385041.69} $\pm$ \phantom{00}\num[group-digits=false, round-mode=figures,round-precision=2]{811.37} & 
\num[group-digits=false, round-mode=figures,round-precision=4]{75827.75} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{314.26} & 
 \num[group-digits=false, round-mode=figures,round-precision=4]{34600.60} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{181.17} \\
Data & 
385052 \phantom {$\pm$ 00000}  & 
75854  \phantom{ $\pm$ 0000}  & 
  34623 \phantom{ $\pm$ 000} \\
\hline\hline
\end{tabular}
}
\end{center}
\end{table}


\begin{table}[!htbp]
\begin{center}
\caption{
\label{tab:event_yields_controlregion2lep_masswindow}
The expected and observed numbers of events for an integrated luminosity of 36.1~fb$^{-1}$ and $\sqrt{s}=$~13~\TeV, shown separately in each \monoWZ 2 lepton control region mass window category. The background yields and uncertainties are shown after the profile likelihood fit to the data (with $\mu = 0$). The quoted background uncertainties include both the statistical and systematic contributions.  The uncertainties in the total background can be smaller than in individual components due to anti-correlations of nuisance parameters.}
\resizebox{\linewidth}{!}{

\begin{tabular}{l cc cc c}
\hline\hline

& \multicolumn{3}{c}{Merged topology, 2 lepton control region $W/Z$ mass window}\\
Process &         
  $0b$  & 
  $1b$  & 
  $2b$ \\
  \hline
  \midrule

$W$+jets & 
 \phantom{.}\num[group-digits=false, round-mode=figures,round-precision=3]{26.23} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{3.39} & 
 \num[group-digits=false, round-mode=figures,round-precision=3]{1.26} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{0.32} & 
 \num[group-digits=false, round-mode=figures,round-precision=2]{0.63} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{0.18}   \\
$Z$+jets & 
 \num[group-digits=false, round-mode=figures,round-precision=3]{4751.50} $\pm$ \phantom{.}\num[group-digits=false, round-mode=figures,round-precision=2]{179.24} & 
 \phantom{.}\num[group-digits=false, round-mode=figures,round-precision=3]{495.14} $\pm$ \phantom{0.}\num[group-digits=false, round-mode=figures,round-precision=2]{55.01}  & 
 \num[group-digits=false, round-mode=figures,round-precision=3]{50.08} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{3.68}   \\
$t\bar{t}$ & 
 \phantom{.}\num[group-digits=false, round-mode=figures,round-precision=3]{48.22} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{4.15}   & 
 \num[group-digits=false, round-mode=figures,round-precision=3]{28.00} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{2.25}   & 
 \num[group-digits=false, round-mode=figures,round-precision=3]{1.71} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{0.44} \\
Single top-quark & 
 \phantom{.}\num[group-digits=false, round-mode=figures,round-precision=3]{4.85} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{ 0.69}  & 
 \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{9.10} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{1.15}   & 
\num[group-digits=false, round-mode=figures,round-precision=3]{1.52} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{0.19} \\
Diboson & 
 \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=3]{240.76} $\pm$ \phantom{0.}\num[group-digits=false, round-mode=figures,round-precision=2]{42.99}  & 
 \num[group-digits=false, round-mode=figures,round-precision=3]{32.66} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{5.82}  & 
 \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{9.09} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{1.78} \\
Total background & 
 \num[group-digits=false, round-mode=figures,round-precision=4]{5071.56} $\pm$ \phantom{0.}\num[group-digits=false, round-mode=figures,round-precision=2]{56.61} & 
 \phantom{.}\num[group-digits=false, round-mode=figures,round-precision=3]{566.17} $\pm$ \phantom{0.}\num[group-digits=false, round-mode=figures,round-precision=2]{15.46}  & 
 \num[group-digits=false, round-mode=figures,round-precision=3]{63.03} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{4.30} \\
Data & 
\phantom{}  5026 \phantom{ $\pm$ 000.} & 
\phantom{}   569 \phantom{ $\pm$ 000.} & 
\phantom{}    66 \phantom{ $\pm$ 000.} \\
  
  
\hline\hline
Process & \multicolumn{3}{c}{Resolved topology, 2 lepton control region $W$/$Z$ mass window}\\
        & $0b$  & $1b$  & $2b$\\
  \midrule

$W$+jets & 
 \phantom{000}\num[group-digits=false, round-mode=figures,round-precision=2]{92.37} $\pm$ \phantom{00}\num[group-digits=false, round-mode=figures,round-precision=2]{11.91} & 
 \phantom{0.}\num[group-digits=false, round-mode=figures,round-precision=2]{8.98} $\pm$ \phantom{.}\num[group-digits=false, round-mode=figures,round-precision=2]{1.93} & 
 \phantom{.}\num[group-digits=false, round-mode=figures,round-precision=2]{0.97} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{0.24} \\
$Z$+jets & 
 \num[group-digits=false, round-mode=figures,round-precision=3]{34452.16} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{1409.68} & 
 \num[group-digits=false, round-mode=figures,round-precision=3]{1963.90} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{197.03} & 
 \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=3]{456.88} $\pm$ \phantom{0.}\num[group-digits=false, round-mode=figures,round-precision=2]{22.52} \\
$t\bar{t}$ & 
 \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=3]{461.66} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{32.87} & 
 \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=3]{496.76}  $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{21.95} & 
 \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=3]{539.32} $\pm$ \phantom{0.}\num[group-digits=false, round-mode=figures,round-precision=2]{16.01} \\
Single top-quark & 
 \phantom{.}\num[group-digits=false, round-mode=figures,round-precision=3]{63.96} $\pm$ \phantom{.}\num[group-digits=false, round-mode=figures,round-precision=2]{5.64}  & 
 \phantom{.}\num[group-digits=false, round-mode=figures,round-precision=3]{56.45} $\pm$ \phantom{.}\num[group-digits=false, round-mode=figures,round-precision=2]{4.65}  & 
 \phantom{.}\num[group-digits=false, round-mode=figures,round-precision=3]{32.06} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{2.55} \\
Diboson & 
 \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{851.99}  $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{147.68} & 
 \phantom{00}\num[group-digits=false, round-mode=figures,round-precision=2]{73.01} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{11.70}  & 
 \phantom{.}\num[group-digits=false, round-mode=figures,round-precision=3]{50.94} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{9.46}\\
Total background & 
\num[group-digits=false, round-mode=figures,round-precision=4]{35922.14} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{186.36} & 
\num[group-digits=false, round-mode=figures,round-precision=4]{2599.10} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{42.89}  & 
\num[group-digits=false, round-mode=figures,round-precision=4]{1080.18} $\pm$ \phantom{0.}\num[group-digits=false, round-mode=figures,round-precision=2]{24.07} \\
Data & 
35947 \phantom { $\pm$ 000}  & 
2570  \phantom{ $\pm$ 000}  & 
1051 \phantom{ $\pm$ 0.00} \\
\hline\hline
\end{tabular}
}
\end{center}
\end{table}

\begin{table}[!htbp]
\begin{center}
\caption{
\label{tab:event_yields_controlregion2lep_sideband}
The expected and observed numbers of events for an integrated luminosity of 36.1~fb$^{-1}$ and $\sqrt{s}=$~13~\TeV, shown separately in each \monoWZ 2 lepton control region mass sideband category. The background yields and uncertainties are shown after the profile likelihood fit to the data (with $\mu = 0$). The quoted background uncertainties include both the statistical and systematic contributions.  The uncertainties in the total background can be smaller than in individual components due to anti-correlations of nuisance parameters.}
\resizebox{\linewidth}{!}{

\begin{tabular}{l cc cc c}
\hline\hline

& \multicolumn{3}{c}{Merged topology, 2 lepton control region $W/Z$ mass sideband}\\
Process &         
  $0b$  & 
  $1b$  & 
  $2b$ \\
  \hline
  \midrule

$W$+jets & 
 \phantom{.}\num[group-digits=false, round-mode=figures,round-precision=3]{14.66}  $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{2.18} & 
 \num[group-digits=false, round-mode=figures,round-precision=3]{2.10} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{0.53} & 
 \num[group-digits=false, round-mode=figures,round-precision=2]{0.60} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{0.12}   \\
$Z$+jets & 
 \num[group-digits=false, round-mode=figures,round-precision=3]{3536.84} $\pm$ \phantom{.}\num[group-digits=false, round-mode=figures,round-precision=2]{143.88} & 
 \phantom{.}\num[group-digits=false, round-mode=figures,round-precision=3]{433.68} $\pm$ \phantom{0.}\num[group-digits=false, round-mode=figures,round-precision=2]{47.64} & 
  \num[group-digits=false, round-mode=figures,round-precision=3]{80.44} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{5.06}  \\
$t\bar{t}$ & 
 \phantom{.}\num[group-digits=false, round-mode=figures,round-precision=3]{36.35} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{2.98}  & 
 \num[group-digits=false, round-mode=figures,round-precision=3]{42.51} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{3.53}  & 
 \num[group-digits=false, round-mode=figures,round-precision=3]{5.41} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{0.66}\\
Single top-quark & 
 \phantom{.}\num[group-digits=false, round-mode=figures,round-precision=3]{4.76} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{0.83}  & 
  \num[group-digits=false, round-mode=figures,round-precision=3]{7.22} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{0.93}  & 
 \num[group-digits=false, round-mode=figures,round-precision=3]{3.29} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{0.58} \\
Diboson & 
 \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=3]{114.41} $\pm$ \phantom{0.}\num[group-digits=false, round-mode=figures,round-precision=2]{22.48}  & 
 \num[group-digits=false, round-mode=figures,round-precision=3]{16.96}  $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{3.13}  & 
  \num[group-digits=false, round-mode=figures,round-precision=3]{4.04} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{0.76} \\
Total background & 
\phantom{} \num[group-digits=false, round-mode=figures,round-precision=4]{3707.01}  $\pm$ \phantom{0.}\num[group-digits=false, round-mode=figures,round-precision=2]{46.55} & 
 \phantom{.}\num[group-digits=false, round-mode=figures,round-precision=3]{502.47} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{13.37} & 
 \num[group-digits=false, round-mode=figures,round-precision=3]{93.79} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{5.28} \\
Data & 
\phantom{} 3696  \phantom{$\pm$ 0.00} & 
\phantom{}  522 \phantom{$\pm$ 0.00}& 
 100 \phantom{$\pm$ 0.00}\\
  
  
\hline\hline
Process & \multicolumn{3}{c}{Resolved topology, 2 lepton control region $W$/$Z$ mass sideband}\\
        & $0b$  & $1b$  & $2b$\\
  \midrule

$W$+jets & 
 \phantom{00}\num[group-digits=false, round-mode=figures,round-precision=3]{266.91} $\pm$ \phantom{00}\num[group-digits=false, round-mode=figures,round-precision=2]{25.14} \phantom{} & 
 \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=3]{21.13} $\pm$ \phantom{.}\num[group-digits=false, round-mode=figures,round-precision=2]{5.27} & 
 \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=3]{3.56} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{0.89} \\
$Z$+jets & 
 \num[group-digits=false, round-mode=figures,round-precision=3]{74606.88} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{3190.36} & 
 \phantom{.}\num[group-digits=false, round-mode=figures,round-precision=3]{5068.30} $\pm$ \num[group-digits=false, round-mode=figures,round-precision=2]{512.79} & 
 \phantom{.}\num[group-digits=false, round-mode=figures,round-precision=4]{1152.28} $\pm$ \phantom{0.}\num[group-digits=false, round-mode=figures,round-precision=2]{49.77} \\
$t\bar{t}$ & 
 \phantom{00}\num[group-digits=false, round-mode=figures,round-precision=3]{806.71} $\pm$ \phantom{00}\num[group-digits=false, round-mode=figures,round-precision=2]{54.70} & 
 \phantom{.}\num[group-digits=false, round-mode=figures,round-precision=4]{1708.31} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{73.02} & 
 \phantom{.}\num[group-digits=false, round-mode=figures,round-precision=4]{1259.87} $\pm$ \phantom{0.}\num[group-digits=false, round-mode=figures,round-precision=2]{38.14 }\\
Single top-quark & 
 \phantom{.}\num[group-digits=false, round-mode=figures,round-precision=4]{104.27} $\pm$ \phantom{0.}\num[group-digits=false, round-mode=figures,round-precision=2]{8.22}  & 
 \num[group-digits=false, round-mode=figures,round-precision=4]{171.47} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{11.83}  & 
 \num[group-digits=false, round-mode=figures,round-precision=4]{106.95} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{7.77} \\
Diboson & 
 \phantom{00}\num[group-digits=false, round-mode=figures,round-precision=2]{865.35} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{164.07} & 
 \phantom{00.}\num[group-digits=false, round-mode=figures,round-precision=2]{94.07} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{15.20}  & 
 \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=3]{16.12} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{2.71} \\
Total background & 
\num[group-digits=false, round-mode=figures,round-precision=4]{76650.12} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{273.58}  & 
\phantom{.}\num[group-digits=false, round-mode=figures,round-precision=4]{7063.29} $\pm$ \phantom{0}\num[group-digits=false, round-mode=figures,round-precision=2]{78.48} & 
\phantom{.}\num[group-digits=false, round-mode=figures,round-precision=4]{2538.78} $\pm$ \phantom{0.}\num[group-digits=false, round-mode=figures,round-precision=2]{43.30} \\
Data & 
76680 \phantom {$\pm$ 0000}  & 
 \phantom{.}7032 \phantom{ $\pm$ 000}  & 
 \phantom{.}2528 \phantom{ $\pm$ 0.00} \\
\hline\hline
\end{tabular}
}
\end{center}
\end{table}


\begin{figure}[!htbp]
\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoWZ/monoV_0lep_0tag_merged_substrFail_massFail_met_XS}}   
\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoWZ/monoV_0lep_1tag_merged_substrFail_massFail_met_XS}}   

\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoWZ/monoV_0lep_0tag_merged_substrPass_massFail_met_XS}}   
\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoWZ/monoV_0lep_1tag_merged_substrPass_massFail_met_XS}}   
\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoWZ/monoV_0lep_2tag_merged_massFail_met_XS}}  

\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoWZ/monoV_0lep_0tag_resolved_massFail_met_XS}}   
\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoWZ/monoV_0lep_1tag_resolved_massFail_met_XS}}   
\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoWZ/monoV_0lep_2tag_resolved_massFail_met_XS}}   
\vskip-0.3cm
\caption{
\label{fig:postfit_sb}
The observed (dots) and expected (histograms) $\met$ distribution obtained with 36.1~\ifb of data in the \monoWZ sideband region after the profile likelihood fit (with $\mu = 0$), shown separately for the (a) $0b$-LP, (b) $1b$-LP, (c) $0b$-HP, (d) $1b$-HP, and (e) $2b$-tag merged-topology event categories and for the (f) $0b$-, (g) $1b$- and (h) $2b$-tag resolved-topology event categories. The total background contribution before the fit to data is shown as a dotted blue line. The hatched area represents the total background uncertainty. The signal expectations for the simplified vector-mediator model with $m_{\chi}=1$~\GeV\ and $m_{Z'}=600$~\GeV\ (dashed red line) and for the invisible Higgs boson decays (dashed blue line) are shown for comparison. The inset at the bottom of each plot shows the ratio of the data to the total post-fit (dots) and pre-fit (dotted blue line) background expectation. 
}
\end{figure}

\begin{figure}[!htbp]
\centering  
\subfigure[]{\includegraphics[width=0.4\textwidth]{pfigures/auxiliary/monoWZ/monoV_1lep_0tag_merged_massPass_met_XS}} 
\subfigure[]{\includegraphics[width=0.4\textwidth]{pfigures/auxiliary/monoWZ/monoV_1lep_0tag_resolved_massPass_met_XS}}
\vskip-0.3cm
\subfigure[]{\includegraphics[width=0.4\textwidth]{pfigures/auxiliary/monoWZ/monoV_1lep_1tag_merged_massPass_met_XS}}
\subfigure[]{\includegraphics[width=0.4\textwidth]{pfigures/auxiliary/monoWZ/monoV_1lep_1tag_resolved_massPass_met_XS}}
\vskip-0.3cm
\subfigure[]{\includegraphics[width=0.4\textwidth]{pfigures/auxiliary/monoWZ/monoV_1lep_2tag_merged_massPass_met_XS}}    
\subfigure[]{\includegraphics[width=0.4\textwidth]{pfigures/auxiliary/monoWZ/monoV_1lep_2tag_resolved_massPass_met_XS}}     
\vskip-0.4cm
\caption{
\label{fig:postfit_1l_merged}
The observed (dots) and expected (histograms) $\metnolep$ distribution obtained with 36.1~\ifb of data in the merged (left) and resolved (right) 1-lepton control region after the profile-likelihood fit (with $\mu = 0$), shown separately for the (a,b) $0b$-, (c,d) $1b$- and (e,f) $2b$-tag categories. The total background contribution before the fit to data is shown as a dotted blue line. The hatched area represents the total background uncertainty. The inset at the bottom of each plot shows the ratio of the data to the total post-fit (dots) and pre-fit (dotted blue line) background expectation. 
}
\end{figure}




\begin{figure}[!htbp]
\centering
\subfigure[]{\includegraphics[width=0.4\textwidth]{pfigures/auxiliary/monoWZ/monoV_2lep_0tag_merged_massPass_met_XS}}
\subfigure[]{\includegraphics[width=0.4\textwidth]{pfigures/auxiliary/monoWZ/monoV_2lep_0tag_resolved_massPass_met_XS}}
\vskip-0.3cm 
\subfigure[]{\includegraphics[width=0.4\textwidth]{pfigures/auxiliary/monoWZ/monoV_2lep_1tag_merged_massPass_met_XS}}
\subfigure[]{\includegraphics[width=0.4\textwidth]{pfigures/auxiliary/monoWZ/monoV_2lep_1tag_resolved_massPass_met_XS}}
\vskip-0.3cm  
\subfigure[]{\includegraphics[width=0.4\textwidth]{pfigures/auxiliary/monoWZ/monoV_2lep_2tag_merged_massPass_met_XS}}     
\subfigure[]{\includegraphics[width=0.4\textwidth]{pfigures/auxiliary/monoWZ/monoV_2lep_2tag_resolved_massPass_met_XS}}     
\vskip-0.4cm
\caption{
\label{fig:postfit_2l_merged}
The observed (dots) and expected (histograms) $\metnolep$ distribution obtained with 36.1~\ifb of data in the merged (left) and resolved (right) 2-lepton control region after the profile-likelihood fit (with $\mu = 0$), shown separately for the (a,b) $0b$-, (c,d) $1b$- and (e,f) $2b$-tag categories. The total background contribution before the fit to data is shown as a dotted blue line. The hatched area represents the total background uncertainty. The inset at the bottom of each plot shows the ratio of the data to the total post-fit (dots) and pre-fit (dotted blue line) background expectation. 
}
\end{figure}








\begin{figure}[!htbp]
\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp_80_0tag_merged_LP}}   
\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp_80_1tag_merged_LP}}   

\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp_80_0tag_merged}}   
\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp_80_1tag_merged}}   
\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp_80_2tag_merged}}  

\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp_80_0tag_resolved}}   
\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp_80_1tag_resolved}}   
\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp_80_2tag_resolved}}   
\vskip-0.3cm
\caption{
\label{fig:postfit_signal_merged_80}
The observed (dots) and expected (histograms) $\met$ distribution obtained with 36.1~\ifb of data at $\sqrt{s}=$~13~\TeV\ in the \monoZprime signal region with $m_{Z'}=$~80~\GeV\ after the profile likelihood fit (with $\mu = 0$), shown separately for the (a) $0b$-LP, (b) $1b$-LP, (c) $0b$-HP, (d) $1b$-HP, and (e) $2b$-tag merged-topology event categories and for the (f) $0b$-, (g) $1b$- and (h) $2b$-tag resolved-topology event categories. The total background contribution before the fit to data is shown as a dotted blue line. The hatched area represents the total background uncertainty. The expectations for the selected dark-Higgs (dashed red line) and dark-fermion (dashed blue line) signal points are shown for comparison. The inset at the bottom of each plot shows the ratio of the data to the total post-fit (dots) and pre-fit (dotted blue line) background expectation. 
}
\end{figure}


\begin{figure}[!htbp]
\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp_100_0tag_merged_LP}}   
\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp_100_1tag_merged_LP}}   

\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp_100_0tag_merged}}   
\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp_100_1tag_merged}}   
\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp_100_2tag_merged}}  

\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp_100_0tag_resolved}}   
\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp_100_1tag_resolved}}   
\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp_100_2tag_resolved}}   
\vskip-0.3cm
\caption{
\label{fig:postfit_signal_merged_100}
The observed (dots) and expected (histograms) $\met$ distribution obtained with 36.1~\ifb of data at $\sqrt{s}=$~13~\TeV\ in the \monoZprime signal region with $m_{Z'}=$~100~GeV after the profile likelihood fit (with $\mu = 0$), shown separately for the (a) $0b$-LP, (b) $1b$-LP, (c) $0b$-HP, (d) $1b$-HP, and (e) $2b$-tag merged-topology event categories and for the (f) $0b$-, (g) $1b$- and (h) $2b$-tag resolved-topology event categories. The total background contribution before the fit to data is shown as a dotted blue line. The hatched area represents the total background uncertainty. The expectations for the selected dark-Higgs (dashed red line) and dark-fermion (dashed blue line) signal points are shown for comparison. The inset at the bottom of each plot shows the ratio of the data to the total post-fit (dots) and pre-fit (dotted blue line) background expectation. 
}
\end{figure}


\begin{figure}[!htbp]
\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp110/monoV_0lep_0tag_resolved_massPass_met_XS}}   \subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp110/monoV_0lep_1tag_resolved_massPass_met_XS}}   \subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp110/monoV_0lep_2tag_resolved_massPass_met_XS}}   

\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp120/monoV_0lep_0tag_resolved_massPass_met_XS}}   \subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp120/monoV_0lep_1tag_resolved_massPass_met_XS}}   \subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp120/monoV_0lep_2tag_resolved_massPass_met_XS}}   

\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp130/monoV_0lep_0tag_resolved_massPass_met_XS}}   \subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp130/monoV_0lep_1tag_resolved_massPass_met_XS}}   \subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp130/monoV_0lep_2tag_resolved_massPass_met_XS}}  
\vskip-0.3cm
\caption{
\label{fig:postfit_signal_resolved_110_130}
The observed (dots) and expected (histograms) $\met$ distribution obtained with 36.1~\ifb of data at $\sqrt{s}=$~13~\TeV\ in the \monoZprime signal region with the resolved event topology after the profile likelihood fit (with $\mu = 0$), shown separately for the (a,d,g) $0b$, (b,e,h) $1b$ and (c,f,i) $2b$-tag event categories, assuming $m_{Z'}$ of (a,b,c) 110~\GeV, (d,e,f) 120~\GeV\ and (g,h,i) 130~\GeV. The total background contribution before the fit to data is shown as a dotted blue line. The hatched area represents the total background uncertainty. The expectations for the selected dark-Higgs (dashed red line) and dark-fermion (dashed blue line) signal points are shown for comparison. The inset at the bottom of each plot shows the ratio of the data to the total post-fit (dots) and pre-fit (dotted blue line) background expectation. 
}
\end{figure}


\begin{figure}[!htbp]
\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp140/monoV_0lep_0tag_resolved_massPass_met_XS}}   \subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp140/monoV_0lep_1tag_resolved_massPass_met_XS}}   \subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp140/monoV_0lep_2tag_resolved_massPass_met_XS}}   

\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp150/monoV_0lep_0tag_resolved_massPass_met_XS}}   \subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp150/monoV_0lep_1tag_resolved_massPass_met_XS}}   \subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp150/monoV_0lep_2tag_resolved_massPass_met_XS}}   

\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp160/monoV_0lep_0tag_resolved_massPass_met_XS}}   \subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp160/monoV_0lep_1tag_resolved_massPass_met_XS}}   \subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp160/monoV_0lep_2tag_resolved_massPass_met_XS}}  
\vskip-0.3cm
\caption{
\label{fig:postfit_signal_resolved_140_160}
The observed (dots) and expected (histograms) $\met$ distribution obtained with 36.1~\ifb of data at $\sqrt{s}=$~13~\TeV\ in the \monoZprime signal region with the resolved event topology after the profile likelihood fit (with $\mu = 0$), shown separately for the (a,d,g) $0b$, (b,e,h) $1b$ and (c,f,i) $2b$-tag event categories, assuming $m_{Z'}$ of (a,b,c) 140~\GeV, (d,e,f) 150~\GeV\ and (g,h,i) 160~\GeV. The total background contribution before the fit to data is shown as a dotted blue line. The hatched area represents the total background uncertainty. The expectations for the selected dark-Higgs (dashed red line) and dark-fermion (dashed blue line) signal points are shown for comparison. The inset at the bottom of each plot shows the ratio of the data to the total post-fit (dots) and pre-fit (dotted blue line) background expectation. 
}
\end{figure}

\clearpage

\begin{figure}[!htbp]
\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp170/monoV_0lep_0tag_resolved_massPass_met_XS}}   \subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp170/monoV_0lep_1tag_resolved_massPass_met_XS}}   \subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp170/monoV_0lep_2tag_resolved_massPass_met_XS}}   

\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp180/monoV_0lep_0tag_resolved_massPass_met_XS}}   \subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp180/monoV_0lep_1tag_resolved_massPass_met_XS}}   \subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp180/monoV_0lep_2tag_resolved_massPass_met_XS}}   

\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp190/monoV_0lep_0tag_resolved_massPass_met_XS}}   \subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp190/monoV_0lep_1tag_resolved_massPass_met_XS}}   \subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp190/monoV_0lep_2tag_resolved_massPass_met_XS}}  
\vskip-0.3cm
\caption{
\label{fig:postfit_signal_resolved_170_190}
The observed (dots) and expected (histograms) $\met$ distribution obtained with 36.1~\ifb of data at $\sqrt{s}=$~13~\TeV\ in the \monoZprime signal region with the resolved event topology after the profile likelihood fit (with $\mu = 0$), shown separately for the (a,d,g) $0b$, (b,e,h) $1b$ and (c,f,i) $2b$-tag event categories, assuming $m_{Z'}$ of (a,b,c) 170~\GeV, (d,e,f) 180~\GeV\ and (g,h,i) 190~\GeV. The total background contribution before the fit to data is shown as a dotted blue line. The hatched area represents the total background uncertainty. The expectations for the selected dark-Higgs (dashed red line) and dark-fermion (dashed blue line) signal points are shown for comparison. The inset at the bottom of each plot shows the ratio of the data to the total post-fit (dots) and pre-fit (dotted blue line) background expectation. 
}
\end{figure}


\begin{figure}[!htbp]
\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp200/monoV_0lep_0tag_resolved_massPass_met_XS}}   \subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp200/monoV_0lep_1tag_resolved_massPass_met_XS}}   \subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp200/monoV_0lep_2tag_resolved_massPass_met_XS}}   

\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp250/monoV_0lep_0tag_resolved_massPass_met_XS}}   \subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp250/monoV_0lep_1tag_resolved_massPass_met_XS}}   \subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp250/monoV_0lep_2tag_resolved_massPass_met_XS}}   

\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp_300_0tag_resolved}}   
\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp_300_1tag_resolved}}   
\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp_300_2tag_resolved}}    
\vskip-0.3cm
\caption{
\label{fig:postfit_signal_resolved_200_350}
The observed (dots) and expected (histograms) $\met$ distribution obtained with 36.1~\ifb of data at $\sqrt{s}=$~13~\TeV\ in the \monoZprime signal region with the resolved event topology after the profile likelihood fit (with $\mu = 0$), shown separately for the (a,d,g) $0b$, (b,e,h) $1b$ and (c,f,i) $2b$-tag event categories, assuming $m_{Z'}$ of (a,b,c) 200~\GeV, (d,e,f) 250~\GeV\ and (g,h,i) 300~\GeV. The total background contribution before the fit to data is shown as a dotted blue line. The hatched area represents the total background uncertainty. The expectations for the selected dark-Higgs (dashed red line) and dark-fermion (dashed blue line) signal points are shown for comparison. The inset at the bottom of each plot shows the ratio of the data to the total post-fit (dots) and pre-fit (dotted blue line) background expectation. 
}
\end{figure}

\begin{figure}[!htbp]
\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp_400_0tag_resolved}}   
\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp_400_1tag_resolved}}   
\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp_400_2tag_resolved}}   

\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp_450_0tag_resolved}}   
\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp_450_1tag_resolved}}   
\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp_450_2tag_resolved}}   

\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp_500_0tag_resolved}}   
\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp_500_1tag_resolved}}   
\subfigure[]{\includegraphics[width=0.32\textwidth]{pfigures/auxiliary/monoZp/mzp_500_2tag_resolved}}    
\vskip-0.3cm
\caption{
\label{fig:postfit_signal_resolved_400_500}
The observed (dots) and expected (histograms) $\met$ distribution obtained with 36.1~\ifb of data at $\sqrt{s}=$~13~\TeV\ in the \monoZprime signal region with the resolved event topology after the profile likelihood fit (with $\mu = 0$), shown separately for the (a,d,g) $0b$, (b,e,h) $1b$ and (c,f,i) $2b$-tag event categories, assuming $m_{Z'}$ of (a,b,c) 400~\GeV, (d,e,f) 450~\GeV\ and (g,h,i) 500~\GeV. The total background contribution before the fit to data is shown as a dotted blue line. The hatched area represents the total background uncertainty. The expectations for the selected dark-Higgs (dashed red line) and dark-fermion (dashed blue line) signal points are shown for comparison. The inset at the bottom of each plot shows the ratio of the data to the total post-fit (dots) and pre-fit (dotted blue line) background expectation. 
}
\end{figure}

